Running a Quantum Circuit at the Speed of Data

We analyze circuits for a number of kernels from popular quantum computing applications, characterizing the hardware resources necessary to take ancilla preparation off the critical path. The result is a chip entirely dominated by ancilla generation circuits. To address this issue, we introduce optimized ancilla factories and analyze their structure and physical layout for ion trap technology. We introduce a new quantum computing architecture with highly concentrated data-only regions surrounded by shared ancilla factories. The results are a reduced dependence on costly teleportation, more efficient distribution of generated ancillae and more than five times speedup over previous proposals.

==> compute_data <==
#!/usr/bin/perl


### constants
$oneQLat = 1;
$twoQLat = 10;
$measLat = 50;
$oneQLatNonTrans = $twoQLat + $measLat + 2 * $oneQLat;
$prepLat = $measLat + $oneQLat;

$moveLat = 1;
$turnLat = 10;

$verifSuccessRate = 0.998;


### subroutines
open(OUT, ">data.tex");

sub printline {
    print OUT "\\newcommand{" . @_[0] . "}{" . @_[1] . "}\n";
}

sub roundToTenth {
    @num = split /\./,@_[0];
    if (scalar(@num) == 1) {
        return @num[0] . ".0";
    } elsif (substr(@num[1],1,1) > "4") {
        if (substr(@num[1],0,1) == "9") {
            return (@num[0]+1) . ".0";
        } else {
            return @num[0] . "." . (1 + substr(@num[1],0,1));
        }
    } else {
        return @num[0] . "." . substr(@num[1],0,1);
    }
}


### Basic physical operation latencies
printline("\\tOneQGate", $oneQLat);
printline("\\tTwoQGate", $twoQLat);
printline("\\tMeas", $measLat);
printline("\\tPhysPrep", $prepLat);
printline("\\tMoveLat", $moveLat);
printline("\\tTurnLat", $turnLat);
printline("\\verifSuccessRate", $verifSuccessRate);



### Stages 2 and 3 for Data Correction Step (all encodings)
### Stage 2: transversal CNOT between data and ancilla; two of them: X and Z
### Stage 3: measure and correct: overlapped
$qecStageTwo = 2 * $twoQLat;
$qecStageThree = $measLat + $oneQLat;
printline("\\qecStageTwo", $qecStageTwo);
printline("\\qecStageThree", $qecStageThree);


### L1 [[7,1,3]]
# Latency for Encoded Zero Ancilla Prepare
$steaneLOneEncZeroPrepLat = $prepLat + $oneQLat + 3 * $twoQLat;
printline("\\steaneLOneEncZeroPrepLat", $steaneLOneEncZeriPrepLat);
# Verification Latency
$steaneLOneVerifyLat = $twoQLat + $measLat;
printline("\\steaneLOneVerify", $steaneLOneVerify);
# Good Prep: Prep 3, verify 2, then use them to X and Z correct; Stages 1 and 3 are overlapped, Stage 2 is not
$steaneLOneGoodEncZeroPrepLat = $steaneLOneEncZeroPrepLat + $steaneLOneVerifyLat + 2 * $twoQLat + $measLat + $oneQLat;
printline("\\steaneLOneGoodEncZeroPrepLat", $steaneLOneGoodEncZeroPrepLat);
# Good QEC Latency
$steaneLOneGoodQECLat = $steaneLOneGoodEncZeroPrepLat + $qecStageTwo + $qecStageThree;
printline("\\steaneLOneGoodQECLat", $steaneLOneGoodQECLat);

### Small Circuit Latencies
printline("\\smallCircuitLat", 2 * $oneQLat + 2 * $twoQLat);
printline("\\smallCircuitLatWQEC", 2 * $oneQLat + 2 * $twoQLat + 2 * $steaneLOneGoodQECLat);

### L2 [[7,1,3]]
$steaneLTwoStageOneTime = 2 * $steaneLOneGoodQECLat - $steaneLOneBasePrep - $steaneLOneVerify;
printline("\\steaneLTwoStageOneTime", $steaneLTwoStageOneTime);
$steaneLTwoTotalTime = $steaneLTwoStageOneTime + $qecStageTwo + $qecStageThree;
printline("\\steaneLTwoTotalTime", $steaneLTwoTotalTime);

### Golay
printline("\\golayTotalTime",0);
printline("\\golayStageOneTime",0);



### Latency numbers for simple circuit in paper
$nonOverlappedQECLat = 2 * $steaneLOneGoodEncZeroPrepLat + 2 * $qecStageTwo + $qecStageThree;
$simpleCircuitLatWithoutQEC = 2 * $oneQLat + 2 * $twoQLat;
$simpleCircuitLatWithQEC = $simpleCircuitLatWithoutQEC + 4 * $nonOverlappedQECLat;
printline("\\nonOverlappedQECLat", $nonOverlappedQECLat);
printline("\\simpleCircuitLatWithoutQEC", $simpleCircuitLatWithoutQEC);
printline("\\simpleCircuitLatWithQEC", $simpleCircuitLatWithQEC);



### Number of unique qubits in each circuit
$qrcaNumQubits = 97;
$qclaNumQubits = 123;
$qftNumQubits = 32;
printline("\\qrcaNumQubits", $qrcaNumQubits);
printline("\\qclaNumQubits", $qclaNumQubits);
printline("\\qftNumQubits", $qftNumQubits);


### Gate breakdown for each circuit
$qrcaTwoQGateCount = 884;
$qrcaOneQTransGateCount = 378;
$qrcaOneQNonTransGateCount = 882;
$qrcaPrepareGateCount = 33;
$qrcaTotalGateCount = $qrcaTwoQGateCount + $qrcaOneQTransGateCount + $qrcaOneQNonTransGateCount + $qrcaPrepareGateCount;
$qrcaOneQNonTransGatePercent = $qrcaOneQNonTransGateCount / $qrcaTotalGateCount;
printline("\\qrcaTwoQGateCount", $qrcaTwoQGateCount);
printline("\\qrcaOneQTransGateCount", $qrcaOneQTransGateCount);
printline("\\qrcaOneQNonTransGateCount", $qrcaOneQNonTransGateCount);
printline("\\qrcaPrepareGateCount", $qrcaPrepareGateCount);
printline("\\qrcaTotalGateCount", $qrcaTotalGateCount);
printline("\\qrcaOneQNonTransGatePercent", roundToTenth (100 * $qrcaOneQNonTransGatePercent));
$qclaTwoQGateCount = 941;
$qclaOneQTransGateCount = 423;
$qclaOneQNonTransGateCount = 987;
$qclaPrepareGateCount = 59;
$qclaTotalGateCount = $qclaTwoQGateCount + $qclaOneQTransGateCount + $qclaOneQNonTransGateCount + $qclaPrepareGateCount;
$qclaOneQNonTransGatePercent = $qclaOneQNonTransGateCount / $qclaTotalGateCount;
printline("\\qclaTwoQGateCount", $qclaTwoQGateCount);
printline("\\qclaOneQTransGateCount", $qclaOneQTransGateCount);
printline("\\qclaOneQNonTransGateCount", $qclaOneQNonTransGateCount);
printline("\\qclaPrepareGateCount", $qclaPrepareGateCount);
printline("\\qclaTotalGateCount", $qclaTotalGateCount);
printline("\\qclaOneQNonTransGatePercent", roundToTenth (100 * $qclaOneQNonTransGatePercent));
$qftTwoQGateCount = 145;
$qftOneQTransGateCount = 4184;
$qftOneQNonTransGateCount = 3816;
$qftPrepareGateCount = 0;
$qftTotalGateCount = $qftTwoQGateCount + $qftOneQTransGateCount + $qftOneQNonTransGateCount + $qftPrepareGateCount;
$qftOneQNonTransGatePercent = $qftOneQNonTransGateCount / $qftTotalGateCount;
printline("\\qftTwoQGateCount", $qftTwoQGateCount);
printline("\\qftOneQTransGateCount", $qftOneQTransGateCount);
printline("\\qftOneQNonTransGateCount", $qftOneQNonTransGateCount);
printline("\\qftPrepareGateCount", $qftPrepareGateCount);
printline("\\qftTotalGateCount", $qftTotalGateCount);
printline("\\qftOneQNonTransGatePercent", roundToTenth (100 * $qftOneQNonTransGatePercent));



##########################################################################################
### Critical paths: not overlapping prepares, but overlapping stages 2 and 3
$qrcaCritPath = $prepLat + 95 * $oneQLat + 381 * $oneQLatNonTrans + 574 * $twoQLat;
$qclaCritPath = 15 * $oneQLat + 51 * $oneQLatNonTrans + 65 * $twoQLat;
$qftCritPath = 1303 * $oneQLat + 1212 * $oneQLatNonTrans + 61 * $twoQLat;
printline("\\qrcaCritPath", $qrcaCritPath);
printline("\\qclaCritPath", $qclaCritPath);
printline("\\qftCritPath", $qftCritPath);

$qrcaQECLatAncPrep = 2 * 1051 * $steaneLOneGoodEncZeroPrepLat;
$qrcaQECLatDataInteract = 2 * 1051 * $qecStageTwo + 1051 * $qecStageThree;
$qclaQECLatAncPrep = 2 * 131 * $steaneLOneGoodEncZeroPrepLat;
$qclaQECLatDataInteract = 2 * 131 * $qecStageTwo + 131 * $qecStageThree;
$qftQECLatAncPrep = 2 * 2576 * $steaneLOneGoodEncZeroPrepLat;
$qftQECLatDataInteract = 2 * 2576 * $qecStageTwo + 2 * 2576 * $qecStageThree;;
printline("\\qrcaQECLatAncPrep", $qrcaQECLatAncPrep);
printline("\\qclaQECLatAncPrep", $qclaQECLatAncPrep);
printline("\\qftQECLatAncPrep", $qftQECLatAncPrep);
printline("\\qrcaQECLatDataInteract", $qrcaQECLatDataInteract);
printline("\\qclaQECLatDataInteract", $qclaQECLatDataInteract);
printline("\\qftQECLatDataInteract", $qftQECLatDataInteract);

printline("\\qrcaCritPathPercentData", roundToTenth(100 * $qrcaCritPath / ($qrcaCritPath + $qrcaQECLatAncPrep + $qrcaQECLatDataInteract)));
printline("\\qclaCritPathPercentData", roundToTenth(100 * $qclaCritPath / ($qclaCritPath + $qclaQECLatAncPrep + $qclaQECLatDataInteract)));
printline("\\qftCritPathPercentData", roundToTenth(100 * $qftCritPath / ($qftCritPath + $qftQECLatAncPrep + $qftQECLatDataInteract)));

printline("\\qrcaCritPathPercentInteract", roundToTenth(100 * $qrcaQECLatDataInteract / ($qrcaCritPath + $qrcaQECLatAncPrep + $qrcaQECLatDataInteract)));
printline("\\qclaCritPathPercentInteract", roundToTenth(100 * $qclaQECLatDataInteract / ($qclaCritPath + $qclaQECLatAncPrep + $qclaQECLatDataInteract)));
printline("\\qftCritPathPercentInteract", roundToTenth(100 * $qftQECLatDataInteract / ($qftCritPath + $qftQECLatAncPrep + $qftQECLatDataInteract)));

printline("\\qrcaCritPathPercentPrep", roundToTenth(100 * $qrcaQECLatAncPrep / ($qrcaCritPath + $qrcaQECLatAncPrep + $qrcaQECLatDataInteract)));
printline("\\qclaCritPathPercentPrep", roundToTenth(100 * $qclaQECLatAncPrep / ($qclaCritPath + $qclaQECLatAncPrep + $qclaQECLatDataInteract)));
printline("\\qftCritPathPercentPrep", roundToTenth(100 * $qftQECLatAncPrep / ($qftCritPath + $qftQECLatAncPrep + $qftQECLatDataInteract)));



### Circuit Runtime if run at the speed of data: anc prep is not counted, but data interaction and syndrome measurement are
$qrcaRuntimeAtSpeedOfData = $qrcaCritPath + $qrcaQECLatDataInteract;
$qclaRuntimeAtSpeedOfData = $qclaCritPath + $qclaQECLatDataInteract;
$qftRuntimeAtSpeedOfData = $qftCritPath + $qftQECLatDataInteract;



##########################################################################################
### Average Encoded Ancilla BW Needed for each circuit for QEC steps only
$qrcaAvgBWNeedForQECLogical = $qrcaTotalGateCount * 2 * 1000 / $qrcaRuntimeAtSpeedOfData;
$qclaAvgBWNeedForQECLogical = $qclaTotalGateCount * 2 * 1000 / $qclaRuntimeAtSpeedOfData;
$qftAvgBWNeedForQECLogical = $qftTotalGateCount * 2 * 1000 / $qftRuntimeAtSpeedOfData;
printline("\\qrcaAvgBWNeedForQECLogical", roundToTenth($qrcaAvgBWNeedForQECLogical));
printline("\\qclaAvgBWNeedForQECLogical", roundToTenth($qclaAvgBWNeedForQECLogical));
printline("\\qftAvgBWNeedForQECLogical", roundToTenth($qftAvgBWNeedForQECLogical));
$qrcaAvgBWNeedForQECPhysical = $qrcaAvgBWNeedForQECLogical * 7;
$qclaAvgBWNeedForQECPhysical = $qclaAvgBWNeedForQECLogical * 7;
$qftAvgBWNeedForQECPhysical = $qftAvgBWNeedForQECLogical * 7;
printline("\\qrcaAvgBWNeedForQECPhysical", roundToTenth($qrcaAvgBWNeedForQECPhysical));
printline("\\qclaAvgBWNeedForQECPhysical", roundToTenth($qclaAvgBWNeedForQECPhysical));
printline("\\qftAvgBWNeedForQECPhysical", roundToTenth($qftAvgBWNeedForQECPhysical));



### Prep time for the simple ancilla factory
$ancFacSimpleLat = $prepLat + 2 * $measLat + 6 * $twoQLat + 2 * $oneQLat + 8 * $turnLat + 30 * $moveLat;
printline("\\ancFacSimpleLat", $ancFacSimpleLat);
printline("\\ancFacSimpleBWLogical", roundToTenth(1000 / $ancFacSimpleLat));



##########################################################################################
### Average Encoded Ancilla BW Needed for each circuit for Non-Transversal Gates only
$qrcaAvgBWNeedForNonTransLogical = $qrcaOneQNonTransGateCount * 1000 / $qrcaRuntimeAtSpeedOfData;
$qclaAvgBWNeedForNonTransLogical = $qclaOneQNonTransGateCount * 1000 / $qclaRuntimeAtSpeedOfData;
$qftAvgBWNeedForNonTransLogical = $qftOneQNonTransGateCount * 1000 / $qftRuntimeAtSpeedOfData;
printline("\\qrcaAvgBWNeedForNonTransLogical", roundToTenth($qrcaAvgBWNeedForNonTransLogical));
printline("\\qclaAvgBWNeedForNonTransLogical", roundToTenth($qclaAvgBWNeedForNonTransLogical));
printline("\\qftAvgBWNeedForNonTransLogical", roundToTenth($qftAvgBWNeedForNonTransLogical));
$qrcaAvgBWNeedForNonTransPhysical = $qrcaAvgBWNeedForNonTransLogical * 7;
$qclaAvgBWNeedForNonTransPhysical = $qclaAvgBWNeedForNonTransLogical * 7;
$qftAvgBWNeedForNonTransPhysical = $qftAvgBWNeedForNonTransLogical * 7;
printline("\\qrcaAvgBWNeedForNonTransPhysical", roundToTenth($qrcaAvgBWNeedForNonTransPhysical));
printline("\\qclaAvgBWNeedForNonTransPhysical", roundToTenth($qclaAvgBWNeedForNonTransPhysical));
printline("\\qftAvgBWNeedForNonTransPhysical", roundToTenth($qftAvgBWNeedForNonTransPhysical));



##########################################################################################
### Average Encoded Ancilla BW Needed for each circuit Overall



##########################################################################################
### Pipelined Ancilla Factory Components
$stageOneArea = 1;
$stageOneHeight = 1;
$stageTwoCNOTArea = 28;
$stageTwoCNOTHeight = 4;
$stageTwoCatArea = 6;
$stageTwoCatHeight = 2;
$stageThreeArea = 10;
$stageThreeHeight = 10;
$stageFourArea = 21;
$stageFourHeight = 21;

$stageOneLat = $prepLat + $oneQLat + $moveLat + 2 * $turnLat;
$stageOneInBWPhysical = 1000 / $stageOneLat;
$stageOneOutBWPhysical = 1000 / $stageOneLat;
printline("\\stageOneLat", $stageOneLat);
printline("\\stageOneInBWPhysical", roundToTenth($stageOneInBWPhysical));
printline("\\stageOneOutBWPhysical", roundToTenth($stageOneOutBWPhysical));
printline("\\stageOneArea", $stageOneArea);

$stageTwoCNOTLat = 3 * $twoQLat + 4 * $turnLat + 5 * $moveLat + 2 * $turnLat;
$stageTwoCNOTInBWPhysical = 1000 * 3 * 7 / $stageTwoCNOTLat;
$stageTwoCNOTOutBWPhysical = 1000 * 3 * 7 / $stageTwoCNOTLat;
printline("\\stageTwoCNOTLat", $stageTwoCNOTLat);
printline("\\stageTwoCNOTInBWPhysical", roundToTenth($stageTwoCNOTInBWPhysical));
printline("\\stageTwoCNOTOutBWPhysical", roundToTenth($stageTwoCNOTOutBWPhysical));
printline("\\stageTwoCNOTArea", $stageTwoCNOTArea);

$stageTwoCatLat = 2 * $twoQLat + 2 * $turnLat + 2 * $moveLat + 2 * $turnLat;
$stageTwoCatInBWPhysical = 1000 * 2 * 3 / $stageTwoCatLat;
$stageTwoCatOutBWPhysical = 1000 * 2 * 3 / $stageTwoCatLat;
printline("\\stageTwoCatLat", $stageTwoCatLat);
printline("\\stageTwoCatInBWPhysical", roundToTenth($stageTwoCatInBWPhysical));
printline("\\stageTwoCatOutBWPhysical", roundToTenth($stageTwoCatOutBWPhysical));
printline("\\stageTwoCatArea", $stageTwoCatArea);

$stageThreeLat = $measLat + $twoQLat + 2 * $moveLat + 2 * $turnLat;
$stageThreeInBWPhysical = 1000 * 10  / $stageThreeLat;
$stageThreeOutBWPhysical = 1000 * 7 * $verifSuccessRate / $stageThreeLat;
printline("\\stageThreeLat", $stageThreeLat);
printline("\\stageThreeInBWPhysical", roundToTenth($stageThreeInBWPhysical));
printline("\\stageThreeOutBWPhysical", roundToTenth($stageThreeOutBWPhysical));
printline("\\stageThreeArea", $stageThreeArea);

$stageFourLat = $measLat + 2 * $twoQLat + 4 * $turnLat + 8 * $moveLat + 2 * $turnLat;
$stageFourInBWPhysical = 1000 * 21 / $stageFourLat;
$stageFourOutBWPhysical = 1000 * 7 / $stageFourLat;
printline("\\stageFourLat", $stageFourLat);
printline("\\stageFourInBWPhysical", roundToTenth($stageFourInBWPhysical));
printline("\\stageFourOutBWPhysical", roundToTenth($stageFourOutBWPhysical));
printline("\\stageFourArea", $stageFourArea);



##########################################################################################
### Final Pipelined Ancilla Factory Stats
$stageOneCount = 24;
$stageTwoCNOTCount = 1;
$stageTwoCatCount = 1;
$stageThreeCount = 3;
$stageFourCount = 2;
printline("\\stageOneCount", $stageOneCount);
printline("\\stageTwoCNOTCount", $stageTwoCNOTCount);
printline("\\stageTwoCatCount", $stageTwoCatCount);
printline("\\stageThreeCount", $stageThreeCount);
printline("\\stageFourCount", $stageFourCount);

$stageOneTotalHeight = $stageOneHeight * $stageOneCount;
$stageTwoCNOTTotalHeight = $stageTwoCNOTHeight * $stageTwoCNOTCount;
$stageTwoCatTotalHeight = $stageTwoCatHeight * $stageTwoCatCount;
$stageTwoTotalHeight = $stageTwoCNOTTotalHeight + $stageTwoCatTotalHeight;
$stageThreeTotalHeight = $stageThreeHeight * $stageThreeCount;
$stageFourTotalHeight = $stageFourHeight * $stageFourCount;
printline("\\stageOneTotalHeight", $stageOneTotalHeight);
printline("\\stageTwoCNOTTotalHeight", $stageTwoCNOTTotalHeight);
printline("\\stageTwoCatTotalHeight", $stageTwoCatTotalHeight);
printline("\\stageTwoTotalHeight", $stageTwoTotalHeight);
printline("\\stageThreeTotalHeight", $stageThreeTotalHeight);
printline("\\stageFourTotalHeight", $stageFourTotalHeight);

$stageOneTotalInBWPhysical = $stageOneInBWPhysical * $stageOneCount;
$stageTwoCNOTTotalInBWPhysical = $stageTwoCNOTInBWPhysical * $stageTwoCNOTCount;
$stageTwoCatTotalInBWPhysical = $stageTwoCatInBWPhysical * $stageTwoCatCount;
$stageThreeTotalInBWPhysical = $stageThreeInBWPhysical * $stageThreeCount;
$stageFourTotalInBWPhysical = $stageFourInBWPhysical * $stageFourCount;
printline("\\stageOneTotalInBWPhysical", roundToTenth($stageOneTotalInBWPhysical));
printline("\\stageTwoCNOTTotalInBWPhysical", roundToTenth($stageTwoCNOTTotalInBWPhysical));
printline("\\stageTwoCatTotalInBWPhysical", roundToTenth($stageTwoCatTotalInBWPhysical));
printline("\\stageThreeTotalInBWPhysical", roundToTenth($stageThreeTotalInBWPhysical));
printline("\\stageFourTotalInBWPhysical", roundToTenth($stageFourTotalInBWPhysical));

$stageOneTotalOutBWPhysical = $stageOneOutBWPhysical * $stageOneCount;
$stageTwoCNOTTotalOutBWPhysical = $stageTwoCNOTOutBWPhysical * $stageTwoCNOTCount;
$stageTwoCatTotalOutBWPhysical = $stageTwoCatOutBWPhysical * $stageTwoCatCount;
$stageThreeTotalOutBWPhysical = $stageThreeOutBWPhysical * $stageThreeCount;
$stageFourTotalOutBWPhysical = $stageFourOutBWPhysical * $stageFourCount;
printline("\\stageOneTotalOutBWPhysical", roundToTenth($stageOneTotalOutBWPhysical));
printline("\\stageTwoCNOTTotalOutBWPhysical", roundToTenth($stageTwoCNOTTotalOutBWPhysical));
printline("\\stageTwoCatTotalOutBWPhysical", roundToTenth($stageTwoCatTotalOutBWPhysical));
printline("\\stageThreeTotalOutBWPhysical", roundToTenth($stageThreeTotalOutBWPhysical));
printline("\\stageFourTotalOutBWPhysical", roundToTenth($stageFourTotalOutBWPhysical));

$stageOneTotalArea = $stageOneArea * $stageOneCount;
$stageTwoCNOTTotalArea = $stageTwoCNOTArea * $stageTwoCNOTCount;
$stageTwoCatTotalArea = $stageTwoCatArea * $stageTwoCatCount;
$stageTwoTotalArea = $stageTwoCNOTTotalArea + $stageTwoCatTotalArea;
$stageThreeTotalArea = $stageThreeArea * $stageThreeCount;
$stageFourTotalArea = $stageFourArea * $stageFourCount;
printline("\\stageOneTotalArea", $stageOneTotalArea);
printline("\\stageTwoCNOTTotalArea", $stageTwoCNOTTotalArea);
printline("\\stageTwoCatTotalArea", $stageTwoCatTotalArea);
printline("\\stageTwoTotalArea", $stageTwoTotalArea);
printline("\\stageThreeTotalArea", $stageThreeTotalArea);
printline("\\stageFourTotalArea", $stageFourTotalArea);

### crossbar area if we use one-column, then two-column, then two-column
$totalCrossbarArea = $stageOneTotalHeight + 2 * $stageThreeTotalHeight + 2 * $stageFourTotalHeight;
$totalComputeArea = $stageOneTotalArea + $stageTwoTotalArea + $stageThreeTotalArea + $stageFourTotalArea;
$totalAncFacArea = $totalCrossbarArea + $totalComputeArea;
printline("\\totalCrossbarArea", $totalCrossbarArea);
printline("\\totalComputeArea", $totalComputeArea);
printline("\\totalAncFacArea", $totalAncFacArea);

### Ancilla Factory final throughput
$totalAncFacBWPhysical = $stageTwoCNOTOutBWPhysical * 0.998 / 3;
$totalAncFacBWLogical = $totalAncFacBWPhysical/ 7;
printline("\\totalAncFacBWPhysical", roundToTenth($totalAncFacBWPhysical));
printline("\\totalAncFacBWLogical", roundToTenth($totalAncFacBWLogical));

### Prints to stdout the factory throughput as limited by each stage
#print $stageOneTotalOutBWPhysical * .998 * 7 / (3 * 10);
#print "\n";
#print $stageTwoCNOTTotalOutBWPhysical * .998 / 3;
#print "\n";
#print $stageTwoCatTotalOutBWPhysical * .998 * 7 / (3 * 3);
#print "\n";
#print $stageThreeTotalOutBWPhysical / 3;
#print "\n";
#print $stageFourTotalOutBWPhysical;
#print "\n";



##########################################################################################
# Pipelined pi/8 ancilla factory stats
$piEightCatPrepArea = 12;
$piEightCatPrepHeight = 6;
$piEightTransXSZArea = 7;
$piEightTransXSZHeight = 7;
$piEightDecodeArea = 12 + 7;
$piEightDecodeHeight = 6 + 7;
$piEightHMTransZArea = 1 + 7;
$piEightHMTransZHeight = 1 + 7;

$piEightCatPrepLat = 7 * $twoQLat + 12 * $turnLat + 8 * $moveLat + 2 * $turnLat;
$piEightCatPrepInBWPhysical = 1000 * 7 / $piEightCatPrepLat;
$piEightCatPrepOutBWPhysical = 1000 * 7 / $piEightCatPrepLat;
printline("\\piEightCatPrepLat", $piEightCatPrepLat);
printline("\\piEightCatPrepInBWPhysical", roundToTenth($piEightCatPrepInBWPhysical));
printline("\\piEightCatPrepOutBWPhysical", roundToTenth($piEightCatPrepOutBWPhysical));
printline("\\piEightCatPrepArea", $piEightCatPrepArea);

$piEightTransXSZLat = 3 * $twoQLat + 3 * $moveLat + 2 * $turnLat;
$piEightTransXSZInBWPhysical = 1000 * 14 / $piEightTransXSZLat;
$piEightTransXSZOutBWPhysical = 1000 * 14 / $piEightTransXSZLat;
printline("\\piEightTransXSZLat", $piEightTransXSZLat);
printline("\\piEightTransXSZInBWPhysical", roundToTenth($piEightTransXSZInBWPhysical));
printline("\\piEightTransXSZOutBWPhysical", roundToTenth($piEightTransXSZOutBWPhysical));
printline("\\piEightTransXSZArea", $piEightTransXSZArea);

$piEightDecodeLat = 7 * $twoQLat + 12 * $turnLat + 8 * $moveLat + 2 * $turnLat;
$piEightDecodeInBWPhysical = 1000 * 14 / $piEightDecodeLat;
$piEightDecodeOutBWPhysical = 1000 * 8 / $piEightDecodeLat;
printline("\\piEightDecodeLat", $piEightDecodeLat);
printline("\\piEightDecodeInBWPhysical", roundToTenth($piEightDecodeInBWPhysical));
printline("\\piEightDecodeOutBWPhysical", roundToTenth($piEightDecodeOutBWPhysical));
printline("\\piEightDecodeArea", $piEightDecodeArea);

$piEightHMTransZLat = $measLat + 2 * $oneQLat + 2 * $moveLat + 2 * $turnLat;
$piEightHMTransZInBWPhysical = 1000 * 8 / $piEightHMTransZLat;
$piEightHMTransZOutBWPhysical = 1000 * 7 / $piEightHMTransZLat;
printline("\\piEightHMTransZLat", $piEightHMTransZLat);
printline("\\piEightHMTransZInBWPhysical", roundToTenth($piEightHMTransZInBWPhysical));
printline("\\piEightHMTransZOutBWPhysical", roundToTenth($piEightHMTransZOutBWPhysical));
printline("\\piEightHMTransZArea", $piEightHMTransZArea);



##########################################################################################
### Final Pipelined pi/8 Ancilla Factory Stats
$piEightCatPrepCount = 4;
$piEightTransXSZCount = 1;
$piEightDecodeCount = 4;
$piEightHMTransZCount = 2;
printline("\\piEightCatPrepCount", $piEightCatPrepCount);
printline("\\piEightTransXSZCount", $piEightTransXSZCount);
printline("\\piEightDecodeCount", $piEightDecodeCount);
printline("\\piEightHMTransZCount", $piEightHMTransZCount);

$piEightCatPrepTotalHeight = $piEightCatPrepHeight * $piEightCatPrepCount;
$piEightCatPrepTotalInBWPhysical = $piEightCatPrepInBWPhysical * $piEightCatPrepCount;
$piEightCatPrepTotalOutBWPhysical = $piEightCatPrepOutBWPhysical * $piEightCatPrepCount;
$piEightCatPrepTotalArea = $piEightCatPrepArea * $piEightCatPrepCount;
printline("\\piEightCatPrepTotalHeight", $piEightCatPrepTotalHeight);
printline("\\piEightCatPrepTotalInBWPhysical", roundToTenth($piEightCatPrepTotalInBWPhysical));
printline("\\piEightCatPrepTotalOutBWPhysical", roundToTenth($piEightCatPrepTotalOutBWPhysical));
printline("\\piEightCatPrepTotalArea", $piEightCatPrepTotalArea);

$piEightTransXSZTotalHeight = $piEightTransXSZHeight * $piEightTransXSZCount;
$piEightTransXSZTotalInBWPhysical = $piEightTransXSZInBWPhysical * $piEightTransXSZCount;
$piEightTransXSZTotalOutBWPhysical = $piEightTransXSZOutBWPhysical * $piEightTransXSZCount;
$piEightTransXSZTotalArea = $piEightTransXSZArea * $piEightTransXSZCount;
printline("\\piEightTransXSZTotalHeight", $piEightTransXSZTotalHeight);
printline("\\piEightTransXSZTotalInBWPhysical", roundToTenth($piEightTransXSZTotalInBWPhysical));
printline("\\piEightTransXSZTotalOutBWPhysical", roundToTenth($piEightTransXSZTotalOutBWPhysical));
printline("\\piEightTransXSZTotalArea", $piEightTransXSZTotalArea);

$piEightDecodeTotalHeight = $piEightDecodeHeight * $piEightDecodeCount;
$piEightDecodeTotalInBWPhysical = $piEightDecodeInBWPhysical * $piEightDecodeCount;
$piEightDecodeTotalOutBWPhysical = $piEightDecodeOutBWPhysical * $piEightDecodeCount;
$piEightDecodeTotalArea = $piEightDecodeArea * $piEightDecodeCount;
printline("\\piEightDecodeTotalHeight", $piEightDecodeTotalHeight);
printline("\\piEightDecodeTotalInBWPhysical", roundToTenth($piEightDecodeTotalInBWPhysical));
printline("\\piEightDecodeTotalOutBWPhysical", roundToTenth($piEightDecodeTotalOutBWPhysical));
printline("\\piEightDecodeTotalArea", $piEightDecodeTotalArea);

$piEightHMTransZTotalHeight = $piEightHMTransZHeight * $piEightHMTransZCount;
$piEightHMTransZTotalInBWPhysical = $piEightHMTransZInBWPhysical * $piEightHMTransZCount;
$piEightHMTransZTotalOutBWPhysical = $piEightHMTransZOutBWPhysical * $piEightHMTransZCount;
$piEightHMTransZTotalArea = $piEightHMTransZArea * $piEightHMTransZCount;
printline("\\piEightHMTransZTotalHeight", $piEightHMTransZTotalHeight);
printline("\\piEightHMTransZTotalInBWPhysical", roundToTenth($piEightHMTransZTotalInBWPhysical));
printline("\\piEightHMTransZTotalOutBWPhysical", roundToTenth($piEightHMTransZTotalOutBWPhysical));
printline("\\piEightHMTransZTotalArea", $piEightHMTransZTotalArea);

### crossbar area if we use two-column, then two-column, then one-column
$piEightTotalCrossbarArea = 2 * $piEightCatPrepTotalHeight + 2 * $piEightDecodeTotalHeight + 2 * $piEightDecodeTotalHeight;
$piEightTotalComputeArea = $piEightCatPrepTotalArea + $piEightTransXSZTotalArea + $piEightDecodeTotalArea + $piEightHMTransZTotalArea;
$piEightTotalArea = $piEightTotalCrossbarArea + $piEightTotalComputeArea;
printline("\\piEightTotalCrossbarArea", $piEightTotalCrossbarArea);
printline("\\piEightTotalComputeArea", $piEightTotalComputeArea);
printline("\\piEightTotalArea", $piEightTotalArea);

### pi/8 Ancilla Factory final throughput
$piEightTotalBWPhysical = $piEightCatPrepTotalOutBWPhysical;
$piEightTotalBWLogical = $piEightTotalBWPhysical/ 7;
printline("\\piEightTotalBWPhysical", roundToTenth($piEightTotalBWPhysical));
printline("\\piEightTotalBWLogical", roundToTenth($piEightTotalBWLogical));

### Prints to stdout the factory throughput as limited by each stage
#print $piEightCatPrepTotalOutBWPhysical;
#print "\n";
#print $piEightTransXSZTotalOutBWPhysical / 2;
#print "\n";
#print $piEightDecodeTotalOutBWPhysical * 7 / 8;
#print "\n";
#print $piEightHMTransZTotalOutBWPhysical;
#print "\n";




##########################################################################################
# Matching BWs
# ancilla generation area for average BW needed
$qrcaDataArea = 7 * $qrcaNumQubits;
$qrcaAvgZeroAncFacArea = ($qrcaAvgBWNeedForQECLogical / $totalAncFacBWLogical) * $totalAncFacArea;
$qrcaAvgPiEightAncFacArea = ($qrcaAvgBWNeedForNonTransLogical / $piEightTotalBWLogical) * $piEightTotalArea +
                            ($qrcaAvgBWNeedForNonTransLogical / $totalAncFacBWLogical) * $totalAncFacArea;
$qrcaAvgTotalAncFacArea = $qrcaAvgZeroAncFacArea + $qrcaAvgPiEightAncFacArea;
$qrcaAvgTotalArea = $qrcaDataArea + $qrcaAvgTotalAncFacArea;
$qrcaAvgAreaPercentData = 100 * $qrcaDataArea / $qrcaAvgTotalArea;
$qrcaAvgAreaPercentZeroAncFac = 100 * $qrcaAvgZeroAncFacArea / $qrcaAvgTotalArea;
$qrcaAvgAreaPercentPiEightAncFac = 100 * $qrcaAvgPiEightAncFacArea / $qrcaAvgTotalArea;
printline("\\qrcaDataArea", $qrcaDataArea);
printline("\\qrcaAvgZeroAncFacArea", roundToTenth($qrcaAvgZeroAncFacArea));
printline("\\qrcaAvgPiEightAncFacArea", roundToTenth($qrcaAvgPiEightAncFacArea));
printline("\\qrcaAvgTotalAncFacArea", roundToTenth($qrcaAvgTotalAncFacArea));
printline("\\qrcaAvgTotalArea", roundToTenth($qrcaAvgTotalArea));
printline("\\qrcaAvgAreaPercentData", roundToTenth($qrcaAvgAreaPercentData));
printline("\\qrcaAvgAreaPercentZeroAncFac", roundToTenth($qrcaAvgAreaPercentZeroAncFac));
printline("\\qrcaAvgAreaPercentPiEightAncFac", roundToTenth($qrcaAvgAreaPercentPiEightAncFac));

$qclaDataArea = 7 * $qclaNumQubits;
$qclaAvgZeroAncFacArea = ($qclaAvgBWNeedForQECLogical / $totalAncFacBWLogical) * $totalAncFacArea;
$qclaAvgPiEightAncFacArea = ($qclaAvgBWNeedForNonTransLogical / $piEightTotalBWLogical) * $piEightTotalArea +
                            ($qclaAvgBWNeedForNonTransLogical / $totalAncFacBWLogical) * $totalAncFacArea;
$qclaAvgTotalAncFacArea = $qclaAvgZeroAncFacArea + $qclaAvgPiEightAncFacArea;
$qclaAvgTotalArea = $qclaDataArea + $qclaAvgTotalAncFacArea;
$qclaAvgAreaPercentData = 100 * $qclaDataArea / $qclaAvgTotalArea;
$qclaAvgAreaPercentZeroAncFac = 100 * $qclaAvgZeroAncFacArea / $qclaAvgTotalArea;
$qclaAvgAreaPercentPiEightAncFac = 100 * $qclaAvgPiEightAncFacArea / $qclaAvgTotalArea;
printline("\\qclaDataArea", $qclaDataArea);
printline("\\qclaAvgZeroAncFacArea", roundToTenth($qclaAvgZeroAncFacArea));
printline("\\qclaAvgPiEightAncFacArea", roundToTenth($qclaAvgPiEightAncFacArea));
printline("\\qclaAvgTotalAncFacArea", roundToTenth($qclaAvgTotalAncFacArea));
printline("\\qclaAvgTotalArea", roundToTenth($qclaAvgTotalArea));
printline("\\qclaAvgAreaPercentData", roundToTenth($qclaAvgAreaPercentData));
printline("\\qclaAvgAreaPercentZeroAncFac", roundToTenth($qclaAvgAreaPercentZeroAncFac));
printline("\\qclaAvgAreaPercentPiEightAncFac", roundToTenth($qclaAvgAreaPercentPiEightAncFac));

$qftDataArea = 7 * $qftNumQubits;
$qftAvgZeroAncFacArea = ($qftAvgBWNeedForQECLogical / $totalAncFacBWLogical) * $totalAncFacArea;
$qftAvgPiEightAncFacArea = ($qftAvgBWNeedForNonTransLogical / $piEightTotalBWLogical) * $piEightTotalArea +
                           ($qftAvgBWNeedForNonTransLogical / $totalAncFacBWLogical) * $totalAncFacArea;
$qftAvgTotalAncFacArea = $qftAvgZeroAncFacArea + $qftAvgPiEightAncFacArea;
$qftAvgTotalArea = $qftDataArea + $qftAvgTotalAncFacArea;
$qftAvgAreaPercentData = 100 * $qftDataArea / $qftAvgTotalArea;
$qftAvgAreaPercentZeroAncFac = 100 * $qftAvgZeroAncFacArea / $qftAvgTotalArea;
$qftAvgAreaPercentPiEightAncFac = 100 * $qftAvgPiEightAncFacArea / $qftAvgTotalArea;
printline("\\qftDataArea", $qftDataArea);
printline("\\qftAvgZeroAncFacArea", roundToTenth($qftAvgZeroAncFacArea));
printline("\\qftAvgPiEightAncFacArea", roundToTenth($qftAvgPiEightAncFacArea));
printline("\\qftAvgTotalAncFacArea", roundToTenth($qftAvgTotalAncFacArea));
printline("\\qftAvgTotalArea", roundToTenth($qftAvgTotalArea));
printline("\\qftAvgAreaPercentData", roundToTenth($qftAvgAreaPercentData));
printline("\\qftAvgAreaPercentZeroAncFac", roundToTenth($qftAvgAreaPercentZeroAncFac));
printline("\\qftAvgAreaPercentPiEightAncFac", roundToTenth($qftAvgAreaPercentPiEightAncFac));






close(OUT);



##########################
# QLA estimates
$QLAAncillaUnitArea = 2 * 7 * 3;
$QLAAncillaUnitsArea = $qftNumQubits * $QLAAncillaUnitArea;


##########################################################################################
# We read in the data files for Execution Time vs. BW Available and output data files
# for execution time vs. total ancilla factory area.
open(OLDDATA, "<graphs/limitedBWAvail32BitRippleZeroLat.dat") or die "computedata must be run from the QISCA08 directory";
open(NEWDATA, ">graphs/ancAreaVsTime32BitRippleZeroLat.dat") or die "computedata must be run from the QISCA08 directory";
while ($line = <OLDDATA>) {
    if (substr($line,0,1) eq "e") {
        print NEWDATA "e\n";
    } else {
        ($QECBWLogicalWanted, $time) = split(" ", $line);
        $piEightBWLogicalWanted = $QECBWLogicalWanted * $qrcaAvgBWNeedForNonTransLogical / $qrcaAvgBWNeedForQECLogical;
        $AncFacArea = ($QECBWLogicalWanted / $totalAncFacBWLogical) * $totalAncFacArea +
                      ($piEightBWLogicalWanted / $piEightTotalBWLogical) * $piEightTotalArea +
                      ($piEightBWLogicalWanted / $totalAncFacBWLogical) * $totalAncFacArea;
        print NEWDATA $AncFacArea . " " . $time . "\n";
    }
}
close(NEWDATA);
close(OLDDATA);
system("gnuplot graphs/ancAreaVsTime32BitRippleZeroLat.gp");

open(OLDDATA, "<graphs/limitedBWAvail32BitCLAZeroLat.dat") or die "computedata must be run from the QISCA08 directory";
open(NEWDATA, ">graphs/ancAreaVsTime32BitCLAZeroLat.dat") or die "computedata must be run from the QISCA08 directory";
while ($line = <OLDDATA>) {
    if (substr($line,0,1) eq "e") {
        print NEWDATA "e\n";
    } else {
        ($QECBWLogicalWanted, $time) = split(" ", $line);
        $piEightBWLogicalWanted = $QECBWLogicalWanted * $qclaAvgBWNeedForNonTransLogical / $qclaAvgBWNeedForQECLogical;
        $AncFacArea = ($QECBWLogicalWanted / $totalAncFacBWLogical) * $totalAncFacArea +
	              ($piEightBWLogicalWanted / $piEightTotalBWLogical) * $piEightTotalArea +
                      ($piEightBWLogicalWanted / $totalAncFacBWLogical) * $totalAncFacArea;
        print NEWDATA $AncFacArea . " " . $time . "\n";
    }
}
close(NEWDATA);
close(OLDDATA);
system("gnuplot graphs/ancAreaVsTime32BitCLAZeroLat.gp");

open(NEWDATA, ">graphs/ancAreaVsTime32BitQFTZeroLat.dat") or die "computedata must be run from the QISCA08 directory";
open(OLDDATA, "<graphs/limitedBWAvail32BitQFTZeroLat.dat") or die "computedata must be run from the QISCA08 directory";
while ($line = <OLDDATA>) {
    if (substr($line,0,1) eq "e") {
        print NEWDATA "e\n";
    } else {
        ($QECBWLogicalWanted, $time) = split(" ", $line);
        $piEightBWLogicalWanted = $QECBWLogicalWanted * $qftAvgBWNeedForNonTransLogical / $qftAvgBWNeedForQECLogical;
        $AncFacArea = ($QECBWLogicalWanted / $totalAncFacBWLogical) * $totalAncFacArea +
	              ($piEightBWLogicalWanted / $piEightTotalBWLogical) * $piEightTotalArea +
                      ($piEightBWLogicalWanted / $totalAncFacBWLogical) * $totalAncFacArea;
        print NEWDATA $AncFacArea . " " . $time . "\n";
    }
}
close(OLDDATA);
close(NEWDATA);


open(OLDDATA, "<graphs/CQLAAncNum32BitQFTZeroLat.dat") or die "computedata must be run from the QISCA08 directory";
$numRegions = 0;
while ($line = <OLDDATA>) {
    if (substr($line,0,1) eq "e") {
        print NEWDATA "e\n";
} elsif ($line =~ /regions: (\d+)/) {
    $numRegions = $1;
    open(NEWDATA, ">graphs/CQLAAncAreaVsTime32BitQFTZeroLat" . $numRegions . "regions.dat") or die "computedata must be run from the QISCA08 directory";
    
    } else {
        ($numAncillaUnits, $time) = split(" ", $line);
        $AncFacArea = $numAncillaUnits * $QLAAncillaUnitArea * $numRegions;
        print "regions " . $numRegions . " area " . $AncFacArea . "\n";
        print NEWDATA $AncFacArea . " " . $time . "\n";
    }
}
close(OLDDATA);
close(NEWDATA);

system("gnuplot graphs/ancAreaVsTime32BitQFTZeroLat.gp");


open(OLDDATA, "<graphs/CQLAAncNum32BitCLAZeroLat.dat") or die "computedata must be run from the QISCA08 directory";
$numRegions = 0;
while ($line = <OLDDATA>) {
    if (substr($line,0,1) eq "e") {
        print NEWDATA "e\n";
} elsif ($line =~ /regions: (\d+)/) {
    $numRegions = $1;
    open(NEWDATA, ">graphs/CQLAAncAreaVsTime32BitCLAZeroLat" . $numRegions . "regions.dat") or die "computedata must be run from the QISCA08 directory";
    
    } else {
        ($numAncillaUnits, $time) = split(" ", $line);
        $AncFacArea = $numAncillaUnits * $QLAAncillaUnitArea * $numRegions;
        print "regions " . $numRegions . " area " . $AncFacArea . "\n";
        print NEWDATA $AncFacArea . " " . $time . "\n";
    }
}
close(OLDDATA);
close(NEWDATA);

system("gnuplot graphs/ancAreaVsTime32BitCLAZeroLat.gp");


open(OLDDATA, "<graphs/CQLAAncNum32BitRippleZeroLat.dat") or die "computedata must be run from the QISCA08 directory";
$numRegions = 0;
while ($line = <OLDDATA>) {
    if (substr($line,0,1) eq "e") {
        print NEWDATA "e\n";
} elsif ($line =~ /regions: (\d+)/) {
    $numRegions = $1;
    open(NEWDATA, ">graphs/CQLAAncAreaVsTime32BitRippleZeroLat" . $numRegions . "regions.dat") or die "computedata must be run from the QISCA08 directory";
    
    } else {
        ($numAncillaUnits, $time) = split(" ", $line);
        $AncFacArea = $numAncillaUnits * $QLAAncillaUnitArea * $numRegions;
        print "regions " . $numRegions . " area " . $AncFacArea . "\n";
        print NEWDATA $AncFacArea . " " . $time . "\n";
    }
}
close(OLDDATA);
close(NEWDATA);

system("gnuplot graphs/ancAreaVsTime32BitRippleZeroLat.gp");


